CAVE-AR: A VR Authoring System to Interactively Design, Simulate, and Debug Multi-user AR Experiences

Despite advances in augmented reality (AR), the process of creating meaningful experiences with this technology is still extremely challenging. Due to different tracking implementations and hardware constraints, developing AR applications either requires low-level programming skills, or is done through specific authoring tools that largely sacrifice the possibility of customizing the AR experience. Existing development workflows also do not support previewing or simulating the AR experience, requiring a lengthy process of trial and error by which content creators deploy and physically test applications in each iteration. To mitigate these limitations, we propose CAVE-AR, a novel virtual reality system for authoring, simulating and debugging custom AR experiences. Available both as a standalone or a plug-in tool, CAVE-AR is based on the concept of representing in the same global reference system both in AR content and tracking information, mixing geographical information, architectural features, and sensor data to simulate the context of an AR experience. Thanks to its novel abstraction of existing tracking technologies, CAVE-AR operates independently of users' devices, and integrates with existing programming tools to provide maximum flexibility. Our VR application provides designers with ways to create and modify an AR application, even while others are in the midst of using it. CAVE-AR further allows the designer to track how users are behaving, preview what they are currently seeing, and interact with them through several different channels. To illustrate our proposed development workflow and demonstrate the advantages of our authoring system, we introduce two CAVEAR use cases in which an augmented reality application is created and tested. We compare the CAVE-AR workflow to traditional development methods and demonstrate the importance of simulation and live application debugging.

==> future.tex <==

\section{Future Work}

%A real-time approach also invites new interaction possibilities from the client's perspective, which include allowing mobile users to modify the virtual content directly from their device.

Our ongoing research is both focused on producing new more quantitative evalutation of our use cases and at the same time on exploring new possible features that our approach makes possible. We plan to further explore new creative AR experiences through the CAVE-AR editor, with particular interest in those involving coordinating users and dynamically assigning tasks directly from inside CAVE2. At the same time, we are exploring the possibility to implement object occlusion without the use of depth maps: since we already have a partial reconstruction of the environment, we can use that one to render content more realistically, showing only the parts that should be visible to the user and hiding or blurring out the ones that are behind walls, for example. Another very important feature we are currently testing involves a further step in the process of making the designer more influence during the execution of an AR experience. Thanks to the tracking system offered by CAVE2, we are able to track the movements of the joints of the designer and render himself \textit{as an avatar inside the virtual scene}, placing him at a desired position. This feature would allow many other interaction possibilities based on a full-body communication between the designer and the users that would see him represented on their mobile phone in front of them, giving advice or indications on how to proceed. Such a form of teleportation would be useful, for instance, for better coordinating tasks or, in the \textit{Riverwalk} example, to guide users and provide them information when they get lost. Similarly, it would be possible to introduce avatars aimed at helping users that are indirectly controlled by the designer and possibly respond to some forms of AI.

Since not everybody can afford to develop an editor application by leveraging a CAVE2, we have ultimately worked on the implementation of some alternative versions of our authoring tool, which aim at maintaining the same main features but with less requirements. Among them, we can currently list the following alternative implementations:

\begin{itemize}
\item Head mounted display (HMD) implementation: basically, this implementation uses the same virtual scene that we presented for CAVE2, but relies on slightly different user interfaces. the designer is completely immersed inside the 3D representation of the real world, to which virtual objects are added, making it easier to recreate the perspective of a user from a first person view. However, the need to stand or seat in a fixed position for eventually prolonged time leads sometimes to fatigue and eye strain due to the excessive use of the HMD display.

\item Unity Editor implementation: this is probably the simplest and cheapest implementation: it leverages the use of Google Maps \cite{googlemaps} and can be performed directly inside Unity Editor, without requiring a complete 3D recontruction of the environment. In this implementation we defined two different views: a \textit{User mode}, a 1:1 scaled simulation where we can preview what the user would be able to see from a particular perspective, and a \textit{Map mode}, a 1:100 scaled map representation with a 3D perspective top-view of the previous mode.

\item Mobile implementation: this implementation is complimentary to the Unity Editor one and provides the possibility to adjust the positioning of content by going onsite and testing overlays directly on top of a live camera feed.

\item Web-based implementation: our idea here is to leverage the huge imagery dataset provided by \textit{Google Street View} \cite{streetview} in order to build an editor that allows the placement of virtual content in 3D inside widely available spherical panoramas, combined with a partial reconstruction of the environment based on depth maps.
\end{itemize}
